Bayesian Framework for Gradient Leakage

Federated learning is an established method for training machine learning models without sharing training data. However, recent work has shown that it cannot guarantee data privacy as shared gradients can still leak sensitive information. To formalize the problem of gradient leakage, we propose a theoretical framework that enables, for the first time, analysis of the Bayes optimal adversary phrased as an optimization problem. We demonstrate that existing leakage attacks can be seen as approximations of this optimal adversary with different assumptions on the probability distributions of the input data and gradients. Our experiments confirm the effectiveness of the Bayes optimal adversary when it has knowledge of the underlying distribution. Further, our experimental evaluation shows that several existing heuristic defenses are not effective against stronger attacks, especially early in the training process. Thus, our findings indicate that the construction of more effective defenses and their evaluation remains an open problem.

==> defense.tex <==
\section{Defending against gradient leakage}

Here we describe proposed defense against gradient leakage in federated learning.

\subsection{Bayes optimal adversary and defense}
\label{sec:bayesopt}

\paragraph{Setup}

Let $\mathcal{X} \subseteq \sR^d$ be an input space, and let $f_\theta: \mathcal{X} \rightarrow \mathcal{Y}$ be a neural network with parameters $\theta$ classifying an input to a label in the label space $\mathcal{Y}$.
We assume that inputs $(x, y)$ are coming from a distribution $\mathcal{D}$ with a marginal distribution $p(x)$.
In standard federated learning, there are $n$ clients with loss functions $l_1, ..., l_n$, who are trying to collaboratively find network parameters $\theta$ which minimize the average loss $\frac{1}{n} \sum_{i=1}^n \E \left[ l_i(\theta, x) \right]$.
In a single training step, each client $i$ first computes $\nabla_{\theta} l_i(\theta, x_i)$ on a batch of data $x_i$, then sends these to the central server that performs gradient descent step to obtain new parameters $\theta' = \theta - \frac{\alpha}{n} \sum_{i=1}^n \nabla_{\theta} l_i(\theta, x_i)$.
To ease the notation, throughout the paper we will assume there is a single client, but same reasoning can be applied for the general case.
We will consider a scenario where each client reports, instead of the true gradient $\nabla_{\theta} l_i(\theta, x_i)$, a noisy gradient $g$ sampled from from a distribution $p_\psi(g|x)$, which we call a defense mechanism, parameterized by $\psi$.
The purpose of the defense mechanism is to add enough noise to hide sensitive user information from the gradients, while retaining high enough informativeness so that it can be used for training.
Naturally, $p(x)$ and $p_\psi(g|x)$ together induce a joint distribution $p(x, g)$.


\paragraph{Adversarial risk}

Assume there is an adversary which can observe the gradient $g$ and is trying to reconstruct the input $x$ that produced this gradient.
Formally, the adversary is a function $f: \sR^k \rightarrow \mathcal{X}$ mapping gradients to inputs.
Given some $(x, g)$ sampled from the joint distribution, adversary will output the reconstruction $f(g)$ and incur some loss $\mathcal{L}(x, f(g))$, where loss is some function $\mathcal{L}: \mathcal{X} \times \mathcal{X} \rightarrow \sR$.
Typically, we will consider binary loss which evaluates to 1 if adversary was not able to reconstruct the original input, and 0 otherwise.
If adversary wants to reconstruct \emph{exact} input $x$, we can define loss to be $\mathcal{L}(x, x') := 1_{x \neq x'}$.
If adversary wants to get to some $\delta$-neighbourhood of the input $x$ in the input space, more appropriate definition of the loss is $\mathcal{L}(x, x') := 1_{d(x, x') > \delta}$.
In this work, we will assume that distance $d$ is simply $l_2$-distance, and later we will discuss possible extensions.
This definition is more useful, especially for image data, because adversary can often get something that is very close the original image in $l_2$ space and reconstruction already contains most of the visual features present in the original image.
Note that if we let $\delta$ approach 0 in the second definition of the loss, we essentially converge to the first loss which can thus be seen as the limit of the second one.
Having defined the loss, we can now define risk of the adversary $f$ as
\begin{equation}
    \label{eq:defrisk}
    R(f) := \E_{x, g} \mathcal{L}(x, f(g)) = \E_{x \sim p(x)} \E_{g \sim p_\psi(g|x)} \mathcal{L}(x, f(g)).
\end{equation}


\paragraph{Bayes optimal adversary}

Let's consider the second definition of the loss for which $\mathcal{L}(x, f(g)) := 1_{||f(g) - x||_2 > \delta}$.
We can then rewrite the definition of the risk as follows:
\begin{align*}
    R(f) &= \E_{x, g} \left[ \mathcal{L}(x, f(g)) \right] \\
         &= \E_g \E_{x|g} \left[ 1_{||x - f(g)||_2 > \delta} \right] \\
         &= \E_g \int_{\mathcal{X}} p(x|g) \cdot 1_{||x - f(g)||_2 > \delta} \,dx \\
         &= \E_g \int_{\mathcal{X} \setminus B(f(g), \delta)} p(x|g) \,dx \\
         &= 1 - \E_g \int_{B(f(g), \delta)} p(x|g) \,dx.
\end{align*}

Here $B(f(g), \delta) := \{x' \in \sR^d, ||x' - f(g)||_2 < \delta\}$ denotes the $l_2$-ball of radius $\delta$ around $f(g)$.
Clearly, the adversary which minimizes the risk, called Bayes optimal adversary, can now be defined as $f(g) := \argmax_{x_0} \int_{B(x_0, \delta)} p(x|g) \,dx$.
Intuitively, adversary predicts $x_0$ which contains the largest amount of probability density in its $\delta$-neighborhood under $l_2$ distance metric.
Note that if we let $\delta \rightarrow 0$, then $f(g) \rightarrow \argmax_{x} p(x|g)$, which would be the solution if we would use the loss that requires recovered input to exactly match the original input.
Function $f$ can now be rewritten using Bayes' rule for $p(x|g)$:
\begin{align}
    f(g) &= \argmax_{x_0 \in \mathcal{X}} \int_{B(x_0, \delta)} p(x|g) \,dx \nonumber \\
        &= \argmax_{x_0 \in \mathcal{X}} \int_{B(x_0, \delta)} \frac{p_\psi(g|x)p(x)}{p(g)} \nonumber \,dx \\
        &= \argmax_{x_0 \in \mathcal{X}} \int_{B(x_0, \delta)} p_\psi(g|x)p(x) \,dx \nonumber \\
        &= \argmax_{x_0 \in \mathcal{X}} \int_{B(x_0, \delta)} \log p_\psi(g|x) + \log p(x) \,dx \label{eq:optadv}
\end{align}

Last two steps are simply multiplying by a constant $p(g)$ and taking logarithm, which both do not affect the argmax.
Given gradient $g$, we now have a way to compute the output $f(g)$ of the Bayes optimal adversary by solving an optimization problem in~\cref{eq:optadv}.

Recall that our goal is to learn a defense mechanism $p_{\psi}(g|x)$ which will add enough noise to remove sensitive information from the gradient, while still providing useful gradients for training.
Formally, assuming that $p_\psi$ is in some parametric family $\mathcal{P}$, in order to hide the information from gradients we have to solve for the parameters $\psi \in \mathcal{P}$ which maximize the risk of the Bayes optimal adversary:
\begin{equation}
  \label{eq:optdef}
  \max_{\psi \in \mathcal{P}} R(f) = \max_{\psi \in \mathcal{P}} 1 - \E_g \int_{B(f(g), \delta)} p_{\psi}(x|g) \,dx  
\end{equation}
Naturally, the above would encourage noise to be as high as possible which would cause training to diverge.
To ensure that noisy gradients are still useful for training, we can require that probability of the original gradients is above a certain threshold, meaning $\E_x \left[ p_{\psi}(\nabla_{\theta} l(\theta, x)) \right] \geq \tau$. In practical implementation of the defense, as described next in~\cref{sec:practice}, we are going to have tradeoff between these two requirements.

\subsection{BAT-GL: Bayesian Adversarial Training against Gradient Leakage}
\label{sec:practice}

In~\cref{sec:bayesopt} we phrased Bayes optimal adversary for reconstructing original data from gradients using an optimization problem in~\cref{eq:optadv}, and the optimal defense which maximizes risk of this Bayes optimal adversary in~\cref{eq:optdef}.
In this section we introduce BAT-GL, standing for Bayesian Adversarial Training against Gradient Leakage, which is practical implementation of these theoretically optimal approaches.

\paragraph{Modeling defense mechanism}

The key component of our defense mechanism is the probability distribution $p_{\psi}(g|x)$ parameterized by $\psi$. In BAT-GL, we are going to use $p_{\psi}(g|x) = \mathcal{N}(\nabla_{\theta}l(\theta, x), \Sigma)$ where $\Sigma$ is a diagonal covariance matrix determined by $\psi$ using $\Sigma_{i,i} = \psi_i$. Using Gaussian distribution gives us a closed form solution for the key quantity $\log p_{\psi}(g|x) = -\frac{1}{2} \sum_{i=1}^n \frac{1}{\psi_i^2} \left( g_i - \left( \nabla_{\theta}l(\theta, x) \right)_i \right)^2 + C$.

\paragraph{Approximating the optimal adversary}

Recall that the optimal adversary $f$ searches for the $\delta$-ball with the maximum value of the integral $\log p_\psi(g|x) + \log p(x)$. We now explain how we can obtain previously proposed attacks by plugging in different approximations for $\log p_\psi(g|x)$ and $\log p(x)$.
Note that the previous calculation shows that Gaussian defense mechanism results in $\log p(g|x)$ which is essentially $l_2$ distance between $g$ and $\nabla_{\theta}l(\theta, x)$ where each component is scaled inversely to its variance.
If we assume that all variances are equal, and that prior is uniform, we recover the loss function from Deep Leakage from Gradients (DLG)~\citep{zhu2019dlg}.
Inverting gradients~\citep{geiping2020inverting} uses a total variation image prior for $\log p(x)$ and then 
measures cosine similarity instead of $l_2$ distance.
GradInversion~\citep{yin2021see} introduces more complex prior based on a combination of total variation, $l_2$ norm of the image and DeepInversion prior.



\begin{table}
  \begin{center}
    \begin{tabular}{lll} 
      \toprule
      Defense & Prior $p(x)$ & Conditional $p_\psi(g|x)$ \\
      \midrule
      DLG & Uniform & Gaussian \\ 
      Inverting Gradients & TV & Cosine \\ 
      GradInversion & TV + $l_2$ + DeepInversion & Gaussian \\ 
      \bottomrule
    \end{tabular}
    \caption{Several existing attacks can be interpreted as instances in our Bayesian framework. We show prior and conditional distribution for corresponding losses that each attack uses.}
    \label{tab:priorwork}
  \end{center}
\end{table}


\red{Need to explain what is the actual adversary used}




\paragraph{Approximating the optimal defense}

Similarly as the optimal attacker is determined by~\cref{eq:optadv}, the optimal parameters for the defense are given by~\cref{eq:optdef}.
Note that~\cref{eq:optdef} requires knowledge of the optimal attacker $f$ which, as we argued earlier, is challenging to compute.
In practice, we will replace the true objective by an approximation.
We can take logarithm of \cref{eq:optdef} and apply Jensen's inequality to obtain the bound:
\begin{equation*}
  \min_{\psi \in \mathcal{P}} \log \E_g \left[ \int_{B(f(g), \delta)} p(x|g) \,dx \right] \geq \min_{\psi \in \mathcal{P}} \E_g \left[ \int_{B(f(g), \delta)} \log p(x|g) \,dx \right]
\end{equation*}
We can then rewrite the lower bound as:
\begin{align}
  \label{eq:approxdef}
  &\min_{\psi \in \mathcal{P}} \E_g \left[ \int_{B(f(g), \delta)} \log p(x|g) \,dx \right] \nonumber \\
  &= \min_{\psi \in \mathcal{P}} \E_g \left[ \int_{B(f(g), \delta)} \left( \log p_{\psi}(g|x) + \log p(x) - \log p(g) \right) \,dx \right] \nonumber \\
  &= \min_{\psi \in \mathcal{P}} \E_g \left[ \int_{B(f(g), \delta)} \left( \log p_{\psi}(g|x) - \log \E_{\tilde{x} \sim p} \left[ p_{\psi}(g|\tilde{x}) \right] \right) \,dx  \right] + C \nonumber \\
  &\approx \min_{\psi \in \mathcal{P}} \E_{g, \tilde{x}} \left[ \int_{B(f(g), \delta)} \left( \log p_{\psi}(g|x) - \log p_{\psi}(g|\tilde{x}) \right) \,dx  \right] + C
\end{align}

\begin{wrapfigure}{R}{0.55\textwidth}
  \begin{minipage}{0.54\textwidth}
    \begin{algorithm}[H]
      \caption{Approximate defense}
      \label{alg:defapprox}
      \begin{algorithmic}
        \STATE $\psi \gets$ defense\_init()
        \FOR{$i=1$ {\bfseries to} $n_{def}$}
        \STATE Sample $(x, y) \sim \mathcal{D}$ \;
        \STATE Sample noisy gradient $g \sim p_{\psi}(g|x)$
        \STATE $x_{att} \gets$ run\_attack($\psi, g$) \;
        \STATE Sample $x_1, ..., x_k$ uniformly from $B(x_{att}, \delta)$ \;
        \STATE $\mathcal{L}(\psi) = \frac{1}{k} \sum_{i=1}^k \log p_{\psi}(g|x) - \log p_{\psi}(g|\tilde{x})$ \;
        \STATE $\psi \gets \psi - \alpha \nabla_{\psi} \mathcal{L}(\psi)$ \;
        \ENDFOR
        \RETURN $\psi$ \;
      \end{algorithmic}
    \end{algorithm}
  \end{minipage}
\end{wrapfigure}


To arrive at the final bound, we first apply Bayes's rule on $p(x|g)$, then use linearity of expectation to move the integration of $p(x)$ outside as it is a constant which does not depend on the parameters $\psi$. Finally, in the last step we use the fact that $p(g) = \E_{\tilde{x} \sim p} \left[ p_{\psi}(g|\tilde{x}) \right]$, and estimate the expectation using a single sample estimate $\tilde{x} \sim p$.
The final expression has an interesting interpretation: we want to find the parameters $\psi$ such that the likelihood of the gradient $g$ is as close as possible for both $x$ in the $\delta$-neighborhood of the reconstruction $f(g)$, and for a randomly sampled $\tilde{x}$ from the prior distribution.


